An Online Probabilistic Distributed Tracing System

Distributed tracing has become a fundamental tool for diagnosing performance issues in the cloud by recording causally ordered, end-to-end workflows of request executions. However, tracing in production workloads can introduce significant overheads due to the extensive instrumentation needed for identifying performance variations. This paper addresses the trade-off between the cost of tracing and the utility of the "spans" within that trace through Astraea, an online probabilistic distributed tracing system. Astraea is based on our technique that combines online Bayesian learning and multi-armed bandit frameworks. This formulation enables Astraea to effectively steer tracing towards the useful instrumentation needed for accurate performance diagnosis. Astraea localizes performance variations using only 10-28% of available instrumentation, markedly reducing tracing overhead, storage, compute costs, and trace analysis time.

==> discussion.tex <==
% \noindent\textbf{Request workflows.}
% Some prior works focus on controlling instrumentation to identify divergence from normal request executions \cite{ArumugaNainar:2010fx,
% Yuan:2012eh, Yuan:2010ww, Zuo:2016et,log20,Liblit:2005dz}.
% For example, Log20 \cite{log20} enables log points to differentiate workflows, aiming to help identify faulty executions.
% % This approach does not apply to our scope. 
% In contrast, Astraea focuses on identifying areas of the code that lead requests’ overall execution to be slow. 
% For example, inefficient implementation of serialization/deserialization might not break functionality, however, can be a significant slowdown \cite{tprof,serde}.
% If workflow information is critical to developers, we envision that the following mitigation techniques can be applied.
% First, Astraea can enable all spans with enforced sampling rates.
% Second, instrumentation necessary to differentiate the workflows (e.g., Log20) can be configured as compulsory in Astraea to be always enabled.
% % Third, tracing clients can be modified to embed the context information of disabled spans to the active spans' tag fields such that workflows can later be reconstructed.

% % \noindent\textbf{Workflows.} 
% % % While distributed tracing is mostly used in performance diagnosis \cite{delimitseer,delimitsage,sambasivan2011diagnosing,vaif,firm}, past research have shown other use cases (e.g., correctness or security) that might require entire workflows \cite{log20, jackpot,ArumugaNainar:2010fx,Yuan:2012eh, Yuan:2010ww, Zuo:2016et,log20,Liblit:2005dz}.
% % % Since Astraea enables (or disables) spans, entire workflows that are useful in other use cases (e.g., fault detection) might not be available for a trace. 
% % We envision that following methods can help mitigate this issue. First, with enforced sampling rates, Astraea can enable all spans.
% % Second, instrumentation that are necessary to differentiate the workflows (such as from Log20 \cite{log20}) can be configured as compulsory in Astraea to be always enabled.
% % Third, tracing clients can be modified to embed the context information of disabled spans to the active spans' tag fields such that entire paths can later be reconstructed. 


% % \noindent\textbf{Adaptive.} Astraea adapts the exponentially weighted mean method (\cite{asd}) that is designed as such that older observations are given lower weights (falling exponentially as the datapoints get older). We use a reasonable default (0.3) but can be configured according to needs.
% % \newpage

% \noindent\textbf{Target systems.} 
% % Astraea applies aggregated trace analysis that are grouped by request types (or endpoints). 
% Astraea targets applications where services (or processes) coordinate to service client requests. 
% Astraea is not designed for applications where the concept of a request is imprecise such as streaming frameworks \cite{timelydataflow}.
We next discuss the scope and limitations of \tool.

\noindent\textbf{Algorithms.} 
% Astraea introduces ABS algorithm to confidently eliminate extraneous instrumentation in traces. 
% Other action elimination algorithms such as Median elimination (ME \cite{me}) or Exponential-gap elimination (EGE \cite{ege}) could also be used for this purpose. 
% We also compared these algorithms with the ABS (\cref{sec:algs}). %(similar to methodology in \cref{sec:apparatus}).
% Results averaged from 20 runs revealed that ABS was able to confidently eliminate 90\% of the spans, while EGE could only halve the set, and ME could not eliminate any of them within 2000 samples.
\tool~ embodies a novel Approximate Bayesian Sampling (ABS) algorithm, built on Bayesian learning and multi-armed bandit frameworks, to accurately eliminate extraneous instrumentation (spans) in traces. 
Action elimination algorithms such as Median elimination (ME \cite{me}) or Exponential-gap elimination (EGE \cite{ege}) also aims to find, with high probability,
optimal arms in the classical multi-armed bandit problem.
We therefore evaluate and compare ABS algorithm with the ME and EGE using production traces (\cref{sec:production}).
The figure reveals that our ABS algorithm makes elimination decisions significantly faster than baselines.
In particular, results averaged from 20 runs revealed that ABS confidently eliminates 90\% of the spans, while EGE could only halve the set, and ME could not eliminate any of them within 2000 samples.
The main advantages of our approach are that 
a) it terminates earlier than alternatives because it requires a much smaller number of samples,
b) does not require fixed sample sizes to make elimination decisions in contrast to alternatives \cite{me,ege}, and % ME and EGE %requires minimum number of samples to make elimination decisions,
c) incorporate batched updates, which is a practical necessity as traces are not available instantaneously.

\begin{figure}[b]
    \includegraphics[width=0.85\columnwidth]{full-files/figures/banditalgs.png}
    \centering
    \caption{Algorithm comparison. Our ABS algorithm makes elimination decisions significantly faster than baselines.}
    \label{fig:utility}
\end{figure}

\noindent\textbf{Root cause vs. localization.}
\tool~ does not claim to infer the root causes.
\tool's primary objective is to enable vital spans to pinpoint problems, reducing costs and improving performance navigation compared to vanilla tracing with a larger number of spans. 
%Astraea catalyzes root cause analysis through span and tag analysis. Astraea continuously reports the ranking of spans based on their utility and records each tag from spans within a dataframe with features corresponding to tags and target is end-to-end latency, and applies Pearson correlation analysis to measure the strength of relationships between.
% Astraea aims to identify locations of the code that cause requests’ execution to be slow. 
Through span and tag analysis, \tool~ can hint at diagnosing performance issues such as implementation bugs, deployments, etc (\cref{sec:cases}).

\noindent\textbf{Statistical sampling approach.}

Request-based sampling is a common practice that randomly selects a subset of requests to trace to reduce costs. \tool~ advances this by enabling per-span sampling decisions at each instrumentation point in addition to request-based sampling decisions made at the start of a request. Both techniques can be used together (sec. 4.4 presents different sampling rates’ impact on diagnosis accuracy and speed). \tool's statistical sampling might miss transient or infrequent problems but can accurately localize persistent performance issues. This is an inherent issue with current tracing standards that use request-based sampling. Our experiments quantified that \tool~ can capture implementation, deployment, and resource-related problems that manifest in 100 to 700 samples while disabling extraneous spans (72-89\%).
\tool's reduced tracing cost opens up the possibility of higher request-based sampling rates and/or expanding instrumentation choices, thereby can enhance problem-capturing capabilities.

% \tool embodies a statistical sampling-based approach to more accurately localize sources of performance issues.
% Longer a problem persists, greater are its chances of manifesting in Astraea samples; 
% however, if a problem does not manifest in a sufficient number of samples, there might be false negatives.
% Our experiments quantify that Astraea helps diagnose various performance issues within $\sim$100-700 samples while disabling extraneous spans.
% Our approach of sampling spans allows for higher request sampling rates, allowing traces of problems to be collected more frequently.

% If a problem does not manifest in a sufficient number of samples collected by Astraea, there might be false negatives

